Semi-supervised Implicit Scene Completion from Sparse LiDAR

Recent advances show that semi-supervised implicit representation learning can be achieved through physical constraints like Eikonal equations. However, this scheme has not yet been successfully used for LiDAR point cloud data, due to its spatially varying sparsity. In this paper, we develop a novel formulation that conditions the semi-supervised implicit function on localized shape embeddings. It exploits the strong representation learning power of sparse convolutional networks to generate shape-aware dense feature volumes, while still allows semi-supervised signed distance function learning without knowing its exact values at free space. With extensive quantitative and qualitative results, we demonstrate intrinsic properties of this new learning system and its usefulness in real-world road scenes. Notably, we improve IoU from 26.3% to 51.0% on SemanticKITTI. Moreover, we explore two paradigms to integrate semantic label predictions, achieving implicit semantic completion. Code and models can be accessed at https://github.com/OPEN-AIR-SUN/SISC.

==> tex/bibliography.tex <==
Let's discuss the fairly mechanical issues of collecting your bibliography, organizing it, and citing prior work. I'd like you to care about the appearance of your References section and about the actual content of the bibliography file. Everybody will see the former and your collaborators will see the latter. You should keep your \bibtex/ source clean and organized for the same reasons that you keep your code clean and organized.

You should adopt and enforce a consistent style for references that are listed in the compiled paper, for \bibtex/ entries, and for citation keys. When I need to find a \bibtex/ source for a given paper, I generally begin with DBLP by searching for ``DBLP Author Name", going to the author's DBLP page, and searching for the paper. The reason is that the DBLP \bibtex/ entires tend to be clean, comprehensive, and accurate. Two things I appreciate is the proper spelling of author names, including special characters, and listing of author names in easily readable and properly punctuated form. For example, compare \texttt{Alex Krizhevsky and Ilya Sutskever and Geoffrey E. Hinton} to \texttt{Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E}. I prefer to look at the former, which is from the DBLP \bibtex/ source~\cite{Krizhevsky2012}, than the latter, which is from Google Scholar for that paper. Google Scholar is in general a poor source for \bibtex/ entries: its entries are often messy, inaccurate, and incomplete. Avoid it. If you can't, check every entry against the paper itself or the information on the journal's or the author's page.

The entry you download from DBLP or another source will usually have too much information and will not be stylistically compatible with other such entries. You should decide for yourself which information you are going to list for conference papers, journal articles, and books. Adopt a specific policy and enforce it consistently, deleting unnecessary information and collecting missing data. For conference papers, my \bibtex/ lists the author, title, booktitle, and year, in that order. That's it. When did you last need the page numbers for a paper? Nobody else needs them either, so don't list them.

For journal articles, I use the author, title, journal, volume, number (if available), and year. You can argue against listing the number and perhaps even the volume (who needs these?), but they take little space and serve to clearly distinguish journal papers from conference papers, so I keep them. For books, I list the author, title, publisher, year, and sometimes the edition~\cite{BlakeZisserman1987}. Refer to examples for citing arXiv reports~\cite{Krizhevsky2014}, institutional technical reports~\cite{Nene1996}, and URLs~\cite{Lichman2013}. Whatever policy you adopt, try to be consistent.

\latex/ has a specific capitalization policy for titles of references. This policy does not always do the right thing. It does not know how to capitalize Euclidean, ConvNet, or 3D. You should do this manually by using curly braces, as shown in the examples~\cite{KrahenbuhlKoltun2011,Krizhevsky2012}.

Adopt a consistent naming scheme for citation keys as well. Your readers will never see them, but you and your collaborators will. This scheme should support easy citation without searching through the \bibtex/ file. To this end, the citation key should in most cases be determined by the author names and the year of publication. Here is my scheme, which you can see implemented in the bibliography of this tutorial. When the paper has two authors, I use both last names and the year, as in \texttt{JordanRumelhart1992}. Otherwise I use the first author's name, as in \texttt{Rumelhart1986}. Only when there are two papers that yield the same citation key according to this scheme do I add something, such as the name of the conference, as in \texttt{PeronaMalik1990:PAMI} and \texttt{PeronaMalik1990:ICCV}, and only when the clash actually arises in the bibliography of the specific paper I am working on. (It rarely does.)

Use a consistent policy for listing the names of conferences and journals as well. When writing for a particular community, I abbreviate the names of conferences and journals that most people in the community will be familiar with, such as NIPS and JMLR in the machine learning community and ICCV and PAMI in computer vision. If the abbreviation may be unfamiliar to a large fraction of the intended audience, I write the full name, such as \texttt{ACM Transactions on Graphics} or \texttt{Conference on Decision and Control}. I try to keep the bibliography clean and skip the \texttt{57th Annual} part.

When most of your citations are in the paper (and again when all of them are in, and one more time before you submit), compile it and read the References section from beginning to end. You will likely notice dozens of little bugs. Fix them and rejoice. You just made the world a better place.

In the paper itself, citations should not interfere with the production of well-formed, readable sentences. Citations are not words and should not be used as such. Refer to backpropagation~\cite{Rumelhart1986} and Krizhevsky et al.~\cite{Krizhevsky2012}, not to~\cite{Rumelhart1986} and~\cite{Krizhevsky2012}.


==> tex/figures.tex <==
\begin{table*}
\centering
\ra{1.05}
\resizebox{1\linewidth}{!}{
	\small
	\begin{tabular}{@{}l@{\hspace{6mm}}*{12}{c@{\hspace{4mm}}}c@{\hspace{8mm}}r@{\hspace{3mm}}r@{}}
		\toprule
		Dataset & $k$-means++ & GMM & fuzzy & MS & AC-C & AC-W & N-Cuts & AP & Zell & SEC & LDMGI & GDL & PIC & RCC & RCC-DR \\
		\midrule
		MNIST & 0.500 & 0.404 & 0.386 & 0.264 & n/a & 0.679 & n/a & 0.478 & n/a & 0.469 & 0.761 & n/a & n/a & \textbf{0.893} & 0.828\\
		COIL-100 & 0.803 & 0.786 & 0.796 & 0.685 & 0.703 & 0.853 & 0.871 & 0.761 & 0.958 & 0.849 & 0.888 & 0.958 & \textbf{0.965} & 0.957 & 0.957 \\
		YTF & 0.783 & 0.793 & 0.769 & 0.831 & 0.673 & 0.801 & 0.752 & 0.751 & 0.273 & 0.754 & 0.518 & 0.655 & 0.676 & 0.836 & \textbf{0.874} \\
		YaleB & 0.615 & 0.591 & 0.066 & 0.091 & 0.445 & 0.767 & 0.928 & 0.700 & 0.905 & 0.849 & 0.945 & 0.924 & 0.941 & \textbf{0.975} & \textbf{0.974} \\
		Reuters & 0.516 & 0.507 & 0.272 & 0.000 & 0.368 & 0.471 & 0.545 & 0.386 & 0.087 & 0.498 & 0.523 & 0.401 & 0.057 & \textbf{0.556} & 0.553 \\
		RCV1 & 0.355 & 0.344 & 0.205 & 0.000 & 0.108 & 0.364 & 0.140 & 0.313 & 0.023 & 0.069 & 0.382 & 0.020 & 0.015 & 0.138 & \textbf{0.442} \\
		Pendigits & 0.679 & 0.695 & 0.695 & 0.694 & 0.525 & 0.728 & 0.813 & 0.639 & 0.317 & 0.741 & 0.775 & 0.330 & 0.467 & 0.848 & \textbf{0.854} \\
		Shuttle & 0.215 & 0.266 & 0.204 & 0.362 & n/a & 0.291 & 0.000 & 0.322 & n/a & 0.305 & \textbf{0.591} & n/a & n/a & 0.488 & 0.513 \\
		Mice Protein & 0.425 & 0.385 & 0.417 & 0.534 & 0.315 & 0.525 & 0.536 & 0.554 & 0.428 & 0.537 & 0.527 & 0.400 & 0.394 & \textbf{0.649} & 0.638 \\
		\midrule
		%\addlinespace[1mm]
		Rank & 7.8 & 8.6 & 9.9 & 9.9 & 12.4 & 6.3 & 6.3 & 8.1 & 10.4 & 7.2 & 4.9 & 9.9 & 10 & 2.4 & \textbf{1.6} \\
		\bottomrule
	\end{tabular}
}
\vspace{1mm}
\caption{Accuracy of all algorithms on all datasets, measured by AMI. Some prior algorithms did not scale to large datasets such as MNIST (70K data points in 784 dimensions). RCC or RCC-DR achieve the highest accuracy on 7 of the 9 datasets. RCC-DR achieves the highest or second highest accuracy on 8 of the 9 datasets. The average rank of RCC-DR across datasets is lower by a multiplicative factor of 3 or more than the average rank of any prior algorithm.}
\label{tab:RCC-results}
%\vspace{-2mm}
\end{table*}

Most figures should be laid out in \latex/. This enables editing captions and adjusting the layout in the tex files themselves without modifying the image files. This may not seem important when you're working on a paper on your own, since you created all the files and can modify them easily, but it becomes critical when collaborating with others. You want your collaborators to be able to revise the captions and adjust the layout without asking you to modify your image files. Another important advantage is that the fonts of the captions are automatically compatible with the rest of the document, are scaled correctly by default, and can be adjusted easily from within the tex file.

There are some exceptions, notably with big compositions that cannot be laid out on a grid or anything close to a grid. An example can be seen in the teaser figure of our work on a large dataset of 3D scans~\cite{Choi2016}. Adjusting the placement of individual images in an external application saved a lot of space and improved the figure. Such exceptional figures can be laid out in an external application such as Illustrator. Having said this, most figures do not fall into this category and we will now discuss the recommended practice of laying out figures in \latex/.

Figure~\ref{fig:teaser} provides an example of convenient figure layout using the tabular environment~\cite{Kundu2016}. The figure is straightforward, take a look at the source. Note that we didn't use \texttt{subfigure}, \texttt{minipage}, or anything of this sort. It's just a table. This gives you maximal flexibility over layout and captions. Figure~\ref{fig:teaser} is also an example of a full-page teaser. Such teaser figures are very common in the graphics community, but were not used in the computer vision community until recently, perhaps because the CVPR/ICCV format didn't seem to allow them. As far as I know, our paper on semantic video segmentation was among the first to use a full-page teaser in a CVPR paper, with the figure reproduced in Figure~\ref{fig:teaser}~\cite{Kundu2016}. Now the dam has broken and the full-page teaser is proliferating.

Figure~\ref{fig:indoor-scenes} provides an example with captions~\cite{Choi2015}. Note again that it's just a table and we have full control over the captions. (For example, we don't have to use (a), (b), etc. We can remove these, replace them with anything we want, adjust their fonts, and so forth.) Figure~\ref{fig:nonrigid} illustrates a trickier case that required some adjustment. Take a look at the source. The cells of the table were moved around such that they actually overlap. This grouped pairs of images and made the figure easier to take in. The color bar on the right is aligned in a multirow cell.

Figure~\ref{fig:DCFlow} provides another example, this time with nice vertically oriented captions on the left and a colorbar aligned in a multicolumn cell at the bottom~\cite{Xu2017}. Note that all figures are laid out using the tabular environment. This environment should be perfectly sufficient for most of your figures.

All figures and tables are centered using the \verb~\centering~ command, not by using the \verb~center~ environment (i.e., \verb~\begin{center}~). The center environment creates unnecessary white space before and after its content. Use the \verb~\centering~ command instead, as demonstrated in the provided examples.

Let us now consider tables. Here the \verb~tabular~ environment is again your friend. It is used in all examples provided here. Before you get fancy, try doing what you want with the tabular environment. It will likely do the job. Table~\ref{tab:RCC-results} provides our first example~\cite{ShahKoltun2017}. Before we talk specifically about this table, we need to talk about table style. You can see that this table has a different style from many tables in technical papers: no vertical lines and very few horizontal lines. I must admit that we had poor table manners in many of our older papers. If you are as clueless about table style as I was for most of my unenlightened professional life, you can set yourself on the path to redemption by reading the documentation for the \texttt{booktabs} package~\cite{Fear2002}. In a nutshell, don't use vertical lines: separate columns with extra space when needed. And use horizontal lines only for specific purposes, as you can see in the examples.


\begin{table*}
\newcolumntype{Z}{S[table-format=2.1,table-auto-round]}
\centering
\ra{1.05}
\small
\begin{tabular}{@{}l@{\hspace{4mm}}*{11}{@{\hspace{4mm}}Z}@{\hspace{8mm}}Z@{}}
  \toprule
  Method & \rot{Building} & \rot{Tree} & \rot{Sky} & \rot{Car} & \rot{Sign} & \rot{Road} & \rot{Pedestrian} & \rot{Fence} & \rot{Pole} & \rot{Sidewalk} & \rot{Bicyclist} & \rot{mean IoU} \\
  \midrule
  SuperParsing & 70.4 & 54.8 & 83.5 & 43.3 & 25.4 & 83.4 & 11.6 & 18.3 & 5.2 & 57.4 & 8.9 & 42.03 \\
  Liu and He & 66.8 & 66.6 & 90.1 & 62.9 & 21.4 & 85.8 & 28 & 17.8 & 8.3 & 63.5 & 8.5 & 47.2 \\
  Tripathi et al. & 74.2 & 67.9 & 91 &  66.5 & 23.6 & 90.7 & 26.2 & 28.5 & 16.3 & 71.9 & 28.2 & 53.18 \\
  Yu and Koltun & 82.6 & 76.2 & 89.9 & 84.0 & 46.9 & 92.2 & 56.3 & 35.8 & 23.4 & 75.3 & 55.5 & 65.3 \\
  Kundu et al. & \bfseries 84 & \bfseries 77.2 & \bfseries 91.3 & \bfseries 85.6 & 49.9 & 92.5 & \bfseries 59.1 & 37.6 & 16.9 & 76.0 & 57.2 & 66.1 \\
  Our result & \bfseries 84.4 & \bfseries 77.5 & \bfseries 91.1 & \bfseries 84.9 & \bfseries 51.3 & \bfseries 94.5 & \bfseries 59 & \bfseries 44.9 & \bfseries 29.5 & \bfseries 82 & \bfseries 58.4 & \bfseries 68.9 \\
  \bottomrule
\end{tabular}
\vspace{1mm}
\caption{Comparison to prior work on the CamVid dataset. We outperform the state-of-the-art system of Kundu et al.~by 2.8 percentage points without utilizing temporal cues.}
\label{tab:PfD}
%  \vspace{-2mm}
\end{table*}


A few notes specifically about Table~\ref{tab:RCC-results}. Take a look at the source and you'll notice a few things. First, we're using the \verb~centering~ command. Second, using the \verb~ra~ macro defined in \verb~vcl-shortcuts~ we are slightly increasing inter-row spacing to improve readability. Third, the table is shrunk to fit the page using the \verb~resizebox~ commands. Then we begin with the \verb~tabular~ environment, with micro-managed inter-column spacing. Make sure you understand every part of the definition of the tabular environment here. The first \verb~@{}~ removes all space to the left of the first column. The first column is left-aligned. It is followed by a space of 6mm, specified by \verb~@{\hspace{6mm}}~. This is followed by 12 identical center-aligned columns with a space of 4mm to the right of each: \verb~*{12}{c@{\hspace{4mm}}}~. Then a center-aligned column followed by an 8mm space: \verb~c@{\hspace{8mm}}~. And finally two right-aligned columns with a space of 3mm between them and no space at the rightmost border of the table: \verb~r@{\hspace{3mm}}r@{}~.


\begin{table}[!htb]
\centering
\ra{1.1}
\resizebox{1\linewidth}{!}{
	\small
	\begin{tabular}{@{}l@{\hspace{6mm}}r@{\hspace{4mm}}r@{\hspace{4mm}}r@{\hspace{4mm}}r@{}}
		\toprule
		Name & Instances & Dimensions & Classes & Imbalance \\
		\midrule
		MNIST & 70,000 & 784 & 10 & $\sim$1 \\
		Coil-100 & 7,200 & 49,152 & 100  & 1 \\
		YaleB & 2,414 & 32,256 & 38  & 1 \\
		YTF & 10,036 & 9,075 & 40 & 13 \\
		Reuters-21578 & 9,082 & 2,000 & 50  & 785 \\
		RCV1 & 10,000 & 2,000 & 4 & 6 \\
		Pendigits & 10,992 & 16 & 10 & $\sim$1 \\
		Shuttle & 58,000 & 9 & 7 & 4,558 \\
		Mice Protein & 1,077 & 77 & 8 & $\sim$1 \\
		\bottomrule
	\end{tabular}
}
\vspace{1mm}
\caption{Datasets used in experiments. For each dataset, the table reports the number of instances, number of dimensions, number of ground-truth clusters, and the imbalance, defined as the ratio of the largest and smallest cardinalities of ground-truth clusters.}
\label{tab:RCC-datasets}
%\vspace{-2mm}
\end{table}


\begin{table*}
\newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\centering
\setlength{\tabcolsep}{3mm}
\ra{1.05}
\small
\begin{tabular}{@{}lccZZZcZZZcr@{}}
  \toprule
  \multirow{2}[3]{*}{Method} & \multirow{2}[3]{*}{\begin{tabular}{l}Domain-\\agnostic\end{tabular}} && \multicolumn{3}{c}{Non-occluded pixels (\%)}  &&  \multicolumn{3}{c}{All pixels (\%)}  && \multirow{2}[3]{*}{Runtime}\\
  \cmidrule(l{3mm}r{3mm}){4-6} \cmidrule(l{3mm}r{3mm}){8-10}
  & && {Fl-bg} & {Fl-fg} & {Fl-all} && {Fl-bg} & {Fl-fg} & {Fl-all} &&  \\
  \midrule
  SOF &  \NoX 	&& 8.11  & 18.16 	& 9.93  &&  14.63	 	& 22.83	& 15.99 && 6 min
  \\
  JFS & \NoX     &&  7.85	& 14.97  &  9.14	&& 15.90	&  19.31	& 16.47 && 13 min
  \\
  SDF &  \NoX 	&& 5.75  & 18.38 	&  8.04  &&  8.61 	& 23.01	& 11.01 && --
  \\
  \midrule
  EpicFlow   & \YesV   &&  15.00	& 24.34  &  16.69	&&  25.81 &  28.69	&  26.29 && 15 sec
  \\
  FullFlow   & \YesV   &&  12.97 	& 20.58  & 14.35 	&& 23.09  &  24.79 	&  23.57 && 4 min
  \\
  CPM-Flow   & \YesV   &&  12.77	& 18.71  & 13.85  	&&  22.32  & 22.81	& 22.40 &&  4.2 sec
  \\
  DiscreteFlow   & \YesV   &&  9.96	& \bfseries 17.03  &  11.25	&&   21.53 & \bfseries 21.76	& 21.57 && 3 min
  \\
  DDF   & \YesV  && 10.44 	& 21.32  & 12.41 	&& 20.36  &  25.19 & 	21.17 && 1 min
  \\
  PatchBatch   & \YesV   &&  10.06	& 22.29  & 12.28 	&&  19.98 & 26.50	& 21.07 && 50 sec
  \\
  DC Flow   & \YesV   &&  \bfseries 8.04 	& 19.84 &  \bfseries 10.18	&&  \bfseries 13.10  &  23.70 	&  \bfseries 14.86 && 8.6 sec
  \\ \bottomrule
\end{tabular}
\vspace{1mm}
\caption{Comparison to state-of-the-art optical flow methods on the KITTI 2015 test set. Our domain-agnostic approach outperforms prior such methods by a significant margin, on both occluded and non-occluded pixels. The presented approach outperforms the most accurate prior method on the main Fl-all measure by 27.7\%. For completeness, we list recent domain-specific methods at the top of the table. The presented approach outperforms two of these methods without using domain-specific information.}
\label{tab:DCFlow-kitti}
%  \vspace{-2mm}
\end{table*}


Table~\ref{tab:RCC-datasets} provides an example of a single-column table from the same paper~\cite{ShahKoltun2017}. It's straightforward. Read the source and make sure you understand everything. Table~\ref{tab:PfD} is a bit more advanced~\cite{Richter2016}. First, it has vertically aligned labels. But more to the point, it uses a special column type from the \verb~siunitx~ package to align numbers at the decimal point. This makes the data easier to parse.

Table~\ref{tab:DCFlow-kitti} is a bit different in that inter-column spacing is controlled by changing the value of \verb~tabcolsep~ and by inserting empty columns when additional space is needed~\cite{Xu2017}. I'm not very happy with this solution because I like the detailed control demonstrated in the previous examples. But inserting additional space using \verb~@{\hspace{l}}~ does not play well with \verb~multicolumn~ cells and I could not find a better solution. Table~\ref{tab:DCFlow-kitti} also provides another example that uses the clever column type from \verb~siunitx~. It also illustrates the use of the helpful \NoX{} and \YesV{} symbols and the use of \verb~cmidrule~, with some trimming for good measure.

Figure~\ref{fig:timing} provides an example of the use of \verb~wrapfig~, taken from our Fast Global Registration paper~\cite{Zhou2016}. This can be particularly useful in single-column layouts with lines that span the width of the page.

\begin{wrapfigure}[10]{r}[0pt]{0.5\linewidth}
\centering
\includegraphics[width=1\linewidth]{figures/FGR/timing.pdf}
\caption{Controlled analysis of the execution time of each step in the algorithm.}
\label{fig:timing}
\end{wrapfigure}
\mypara{Captions.}
The general rule is that captions should stand on their own. A casual reader should be able to look at a figure, read the caption, and understand what is being shown. The reader should not have to hunt for the explanation in the text. The figure with its caption should be as self-contained and self-explanatory as possible. More broadly, a common guideline is that the reader should be able to understand the paper at a high level by simply examining the figures and reading their captions. A reader who picks your paper up for the first time should be able to look at the first figure and read its caption, then the second figure and so on, and get a pretty good sense of the paper after they are done. Ideally, they should not be stymied by figures that are impossible to understand because the captions do not actually explain the content.

This guideline can be useful in suggesting figures that your paper may be lacking. Is there a key component of your approach or a particularly important experiment that can be visually illustrated? Will a casual reader miss something important without this illustration, something you want everybody to see? Then add a figure for this important concept, stage, or experiment.

Captions often have a specific structure. First, a phrase or a sentence that summarize the content of the figure. The title of the figure, if you will. In Table~\ref{tab:DCFlow-kitti}, for example, this is \emph{``Comparison to state-of-the-art optical flow methods on the KITTI 2015 test set.''} Next, a detailed explanation of the content. This is usually the bulk of the caption and often has a structure such as \emph{``From left to right, ...''} or \emph{``(a) ... . (b) ... . etc.''}. Finally, the upshot, the take-away.

Not all captions have all three parts. Sometimes the middle part -- detailed explanation of the content -- is not needed. In Table~\ref{tab:DCFlow-kitti}, the middle part is omitted and the caption mostly consists of a long take-away. In Table~\ref{tab:RCC-datasets}, there is no take-away, just a mechanical explanation of the content. The first part -- the ``title'' -- should almost always be present.

\mypara{Figure placement.}
There are two general guidelines that you should follow. First, figures should appear in order. Figure 7 should not appear before Figure 5. \latex/ will break this guideline if you are not careful. You should notice and fix inversions when they occur. Second, figures should generally be referred to on or before the page on which they appear. This guideline often needs to be broken, but try to adhere to it as much as possible.


==> tex/notation.tex <==
Adopt clean and consistent notation. Think about your notation, it's important. In general, you want to introduce notation for entities that are referred to multiple times and need to be precisely identified. If at any point you're writing ``we then add the vector we have just obtained to the vector we have obtained previously", you need to define notation. Think of it in terms of compiling your text in the reader's mind. Does your text compile deterministically and unambiguously? Will every reader understand exactly what you are referring to or is there vagueness that can lead to two plausible and incompatible representations in different readers' minds? Or simply a sense of unease because the reader thinks they probably know which vector you are referring to but is not quite sure because you weren't sufficiently precise? You need to define notation that lets your paper compile unambiguously in the reader's mind.

Your notation should be consistent, such that even its form helps the reader understand what you are doing and reminds the reader what is being referred to. I generally use bold lower-case letters for vectors ($\xx$, $\yy$, $\zz$) and bold upper-case letters for matrices and tensors ($\XX$, $\TT$, $\VV$). Functions are generally upper-case ($E$, $F$), sets are upper-case calligraphic ($\aA$, $\sS$), and constants are lower-case and sometimes Greek ($a$, $k$, $\lambda$, $\gamma$). These are not ironclad rules and I have violated them many times. Try to be consistent and always try to help the reader understand exactly what you are doing, while being as direct as possible.

The enclosed \texttt{vcl-shortcuts.tex} file provides many useful definitions that make your \latex/ source easier to write, read, and edit. We use them for all papers in the lab. Let's look at some examples that illustrate the use of these definitions. We begin with a fragment from Section 3.1 of one of our papers on dense random fields~\cite{KraehenbuehlKoltun2013}.

\vspace{3ex}
\hrule
\vspace{0.5ex}
We begin by rewriting the KL divergence in vector notation:
\begin{equation}
\resizebox{.9\hsize}{!}{$\displaystyle{
D(Q\|P) = \underbrace{\qq\trans \log \qq}_\text{entropy} + \underbrace{\qq\trans \uu + \frac{1}{2}\qq^\top \Psi \qq + \log Z(\II,\btheta)}_\text{cross entropy},
}$}
\label{eq:KL-vec}
\end{equation}
where $\qq$ and $\uu$ are vectors of length $N\timess M$ with elements ${\qq_{(i,l)} = Q_i(X_i=l)}$ and ${\uu_{(i,l)} = \psi_i( X_i = l )}$, respectively.
\vspace{1pt}
\hrule
\vspace{3ex}

Read the source of this fragment. Note how much more concise and readable it is due to the definitions in \texttt{vcl-shortcuts.tex}. My definitions are not optimal, but they can be used as a starting point. They lubricate collaboration in the lab because we don't need to keep readjusting to different conventions.

The fragment around equation (\ref{eq:KL-vec}) illustrates a number of additional points. First, you can proportionately shrink equations that would otherwise overflow. Use this superpower sparingly. It is usually better to break an equation up into multiple lines than to shrink it. If the resized equation is visibly different from others around it, don't resize unless breaking the equation would be even worse. Second, you can prevent \latex/ from breaking up inline math by putting curly braces inside the dollar signs: use \verb~${x+y+z}$~ as opposed to \verb~$x+y+z$~ for longer inline expressions that you want to keep in a single line. Third, I don't like the amount of space around the default \verb~$\times$~ operator and use a custom one, \verb~$\timess$~. Except in superscripts and subscripts, where the default \verb~$\times$~ looks better.

Here is a fragment from a different work.

\vspace{3ex}
\hrule
\vspace{0.5ex}
We train a convolutional network to classify an image into one of the 116 classes in the dataset. Let ${\dD = \{\xx_i,y_i\}_i}$ be the training set, such that $\xx_i$ is an image and $y_i \in \cC$ is a class label. The convolutional network is a parameterized function approximator, denoted by $f(\cdot;\btheta)$, where $\btheta$ are the parameters. The network $f$ maps from the space of images to the space $\Re^{|\cC|}$. Let $f_y(\xx;\btheta)$ be the $y^{\text{th}}$ element of the vector $f(\xx;\btheta)$. Given the data $\dD$, the goal is to optimize the parameters $\btheta$ such that $f_{y_i}(\xx_i;\btheta)$ is maximized relative to all other elements $f_y(\xx_i;\btheta)$. We use the cross-entropy loss:
\begin{equation*}
	\lL(\btheta) = \sum_i \left( -f_{y_i}(\xx_i;\btheta) + \log \sum_y \exp\big(f_{y}(\xx_i;\btheta)\big) \right).
\end{equation*}
\vspace{0.5ex}
\hrule
\vspace{3ex}

A few notes about this one. First, I violated my own rule about using upper-case calligraphic letters for sets in order to denote the loss by the nice symbol $\lL$. (Yes, I do feel a tinge of remorse.) Second, this equation fits into a line when it's not numbered. When it's numbered, the number is pushed onto the next line. Given how nice this one is on a single line, I would shrink it slightly to make space for the number rather than break the equation up.

Let's use a couple of additional examples from the dense random fields paper to illustrate alignment and some additional tricks.

\vspace{3ex}
\hrule
\vspace{0.5ex}
CCCP leads to the following optimization problem:
\begin{alignat}{2}
& \underset{\qq}{\minimize}\quad &&
\qq\trans \log \qq + \qq\trans \ee^{(t)} - \frac{1}{2} \sum_{m=1}^C \qq\trans \II_N \otimes \bmu^{(m)} \qq \notag\\
& \text{subject to}\quad &&
\bOne\trans \qq_i = 1 \quad \text{for}\ i=1,\ldots,N \label{eq:CCCP}
\end{alignat}
where $\ee^{(t)} = \nabla g( \qq^{(t-1)} )$. The entropy term $\qq\trans \log \qq$ restricts the domain of $\qq$ to non-negative values. This makes an explicit constraint $\qq \ge 0$ redundant.

In the mean field optimization problem (\ref{eq:CCCP}), each marginal $\qq_i$ is independent of every other marginal $\qq_j$. We minimize each marginal $\qq_i$ independently. The Karush-Kuhn-Tucker (KKT) conditions are
\begin{align}
 \log \qq_i^{(t)} - \left(\sum_{m=1}^C\bmu^{(m)}\right) \qq_i^{(t)} + \lambda \bOne + \ee_i^{(t)} &= \bZero \notag\\
 \bOne\trans \qq_i^{(t)} &= 1. \label{eq:KKT}
\end{align}
Strong duality holds since the objective in (\ref{eq:CCCP}) is convex and continuously differentiable, and the constraints are affine. This means that a solution to the KKT conditions (\ref{eq:KKT}) minimizes the objective (\ref{eq:CCCP}).

The derivative of the KKT conditions with respect to the model parameters yields a set of linear constraints on the gradient of each marginal:
\begin{align}
 \diag\left( \frac{1}{\qq_i^{(t)}} \right) \frac{\partial \qq_i^{(t)}}{\partial \btheta} &= - \frac{\partial \lambda}{\partial \btheta} \bOne - \frac{\partial \ee_i^{(t)}}{\partial \btheta} \notag\\
 \bOne\trans \frac{\partial \qq_i^{(t)}}{\partial \btheta} &= 0. \label{eq:grad-KKT}
\end{align}
As shown in supplementary material, the linear system (\ref{eq:grad-KKT}) is full rank and invertible. The gradient $\frac{\partial \qq_i^{(t)}}{\partial \btheta}$ is thus always well-defined and is given by
\begin{equation}
 \frac{\partial \qq_i^{(t)}}{\partial \btheta} = \AA^{(t)}_i \frac{\partial \ee_i^{(t)}}{\partial \btheta},
\label{eq:grad-simple}
\end{equation}
where $\AA^{(t)}_i = \qq_i^{(t)}\qq_i^{(t)\top} - \diag\left(\qq_i^{(t)}\right)$.
%For notational convenience let $\AA^{(t)}$ be the block diagonal matrix with blocks $\AA^{(t)}_i$, for $i=1,\ldots, N$.
\vspace{0.5ex}
\hrule
\vspace{3ex}

As you may have noticed, I treat equations as parts of sentences. When a new sentence begins after an equation, I generally put a period at the end, as in the case of equation~(\ref{eq:grad-KKT}). Otherwise I use a comma or nothing at all, depending on the structure of the surrounding sentence, as in the case of equation (\ref{eq:grad-simple}). But you don't have to fret about this and you can see that I break these rules myself, for example in equation (\ref{eq:CCCP}). (Can you spot the infraction?)

Here is a fragment from our paper on optical flow~\cite{Xu2017}, illustrating alignment of the long triplet loss.

\vspace{3ex}
\hrule
\vspace{0.5ex}
We train a convolutional network ${f:\Re^{9\times 9} \rightarrow \Re^d}$ that embeds input patches into the feature space. Let $\btheta$ be the parameters of the network. Let ${\dD = \{(\xx_{i}^{a}, \xx_{i}^{p}, \xx_{i}^{n})\}_{i}}$ be a set of triplets of patches such that $\xx_{i}^{a}$ is known to be more similar to $\xx_{i}^{p}$ than to $\xx_{i}^{n}$, for all $i$. We optimize the embedding using the triplet loss:
\begin{alignat}{1}
\lL(\btheta) = \frac{1}{|\dD|} \sum_{i=1}^{|\dD|} \big[ m & + \norm{f(\xx_{i}^{a};\btheta) - f(\xx_{i}^{p};\btheta) }^2 \notag\\
& - \norm{ f(\xx_{i}^{a};\btheta) - f(\xx_{i}^{n};\btheta)}^2 \big]_{+}.
\label{eq:triplet}
\end{alignat}
\hrule
\vspace{3ex}

Finally, here is an algorithm from the dense random fields paper we've used for most of this section~\cite{KraehenbuehlKoltun2013}.

\begin{algorithm}[h]
\caption{Mean field gradient}
\label{alg:MFG}
\begin{algorithmic}[1]
  \For{$t=1$ {\bfseries to} $n$} \label{line:inference_start}
    \State Run inference to compute $\qq^{(t)}$
  \EndFor \label{line:inference_end}
  \State $\bb^{(n)} \gets \AA^{(n)} \left(\nabla L(\qq^{(n)})\right)\trans$ \label{line:back_inference_start}
  \For{$t=n-1$ {\bfseries to} $1$}
    \State $\bb^{(t)} \gets \AA^{(t)} \hat\Psi \bb^{(t+1)}$ \Comment{Message passing}
  \EndFor \label{line:back_inference_end}
  \State $\gg \gets \bZero$
  \For{$t=1$ {\bfseries to} $n$}
    \State $\gg \gets \gg + \frac{\partial \bb^{(t)\top} \uu}{\partial \btheta}$ \Comment{Unary gradient} \label{line:unary_grad}
    \State $\gg \gets \gg + \frac{\partial \bb^{(t)\top} \hat\Psi \qq^{(t)}}{\partial \btheta}$ \Comment{Pairwise gradient} \label{line:pairwise_grad}
  \EndFor
  \State $\frac{\partial L(\qq^{(n)})}{\partial \btheta} \gets \gg$
\end{algorithmic}
\end{algorithm}


==> tex/overview.tex <==


\begin{figure*}[t]
\centerline{\includegraphics[width=1\textwidth]{figures/main.pdf}}
\vspace{2mm}
\caption{\textbf{Overview of viewpoint SCSNet.} Given an input 3D occupancy volume, the discriminative model firstly maps it into the corresponding shape embedding volume with two sparse network and a coarse SSC volume with a bypass dense network. Then, a differentiable trilinear sampling module and a positional encoding module are exploited to obtain pointwise shape embeddings and encoded coordinates for sampled points. Finally, the sampled pointwise shape embeddings and encoded coordinates are concatenated together and fed into the generative model, where an implicit conditional SIREN is employed to predict SDF values of the sampled points. }
\label{fig:mainfig}
\end{figure*}
We firstly propose a hybrid neural network architecture named SEISMIC, combining a sparse convolutional network (as a discriminative model) with a generative model. 

The pipeline of the SCSNet is illustrated in Fig.~\ref{fig:mainfig}. It is composed of four main parts: 1) \textbf{Discriminative Model}; 2) \textbf{Differentiable Trilinear Sampling Module}; 3) \textbf{Positional Encoding Module}; 4) \textbf{Generative Model}.

Taking an incomplete point cloud $P_{\rm{Li}} \in \mathbb{R}^{N_{\rm{Li}}\times3}$ as input, the network firstly conducts voxelization to obtain 3D volume $V_{\rm{occ}}$. Then the discriminative model $f_d$ maps it into a shape embedding volume $V_{\rm{SE}}$ and a coarse SSC volume $V_{\rm{SSC}}$:
\begin{equation}
f_d(V_{\rm{occ}}) = (V_{\rm{SE}}, V_{\rm{SSC}}).
\end{equation}
The dimension of voxel-wise shape embedding is $d_{\rm{se}}$, and SSC voxel output has $C+1$ channels, which denotes the count of semantic categories with a special non-object one. Then a positional encoding module $f_{\rm{enc}}$ is proposed to turn the 3D-cartesian coordinates $\bm x_i$ of ${p_i}$ into a $d_{\rm{enc}}$ dimensional representation $\bm y_i$:
\begin{equation}
f_{\rm{enc}}(\bm x_i) = \bm y_i: \bm x_i \in \mathbb{R}^{3}, \bm y_i \in \mathbb{R}^{d_{\rm{enc}}}.
\end{equation}
Simultaneously, the differentiable trilinear sampling module $f_{\rm{tri}}$ samples the pointwise shape embeddings $\bm e_i$ for ${p_i}$ from shape embedding volume $V_{\rm{SE}}$ using trilinear interpolation:
\begin{equation}
f_{\rm{tri}}(\bm x_i, V_{\rm{SE}}) = \bm e_i: \bm x_i \in \mathbb{R}^{3}, \bm e_i \in \mathbb{R}^{d_{\rm{se}}}.
\end{equation}

After that, taking the concatenated feature $[\bm y_i, \bm e_i]$ as input, the signed distance function (SDF) value of every points from $P$ in the domain $\Omega$ can be implicitly represented by the generative model $f_g$:
\begin{equation}
f_g([\bm y_i, \bm e_i]) \approx {\rm{SDF}}(\bm x_i), \forall \bm x_i \in \Omega.
\end{equation}
Finally, by extracting the iso-points from the implicit neural surface where SDF values are equal to zero, and leveraging KNN searching method to query labels from the coarse SSC results $V_{\rm{SSC}}$, the final fine SSC results at any resolution can be predicted.

